ET-SEED: Efficient Trajectory-Level SE(3) Equivariant Diffusion Policy

Imitation learning, e.g., diffusion policy, has been proven effective in various robotic manipulation tasks. However, extensive demonstrations are required for policy robustness and generalization. To reduce the demonstration reliance, we leverage spatial symmetry and propose ET-SEED, an efficient trajectory-level SE(3) equivariant diffusion model for generating action sequences in complex robot manipulation tasks. Further, previous equivariant diffusion models require the per-step equivariance in the Markov process, making it difficult to learn policy under such strong constraints. We theoretically extend equivariant Markov kernels and simplify the condition of equivariant diffusion process, thereby significantly improving training efficiency for trajectory-level SE(3) equivariant diffusion policy in an end-to-end manner. We evaluate ET-SEED on representative robotic manipulation tasks, involving rigid body, articulated and deformable object. Experiments demonstrate superior data efficiency and manipulation proficiency of our proposed method, as well as its ability to generalize to unseen configurations with only a few demonstrations. Website: https://et-seed.github.io/

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tex/Derivation.tex <==
\section{\SE group and \se algebra}
\label{appd:SE&se}

\subsection{Basic Terms}
An element in $SE(3)$ can be represented as a $4\times 4$ matrix

\begin{equation}
\begin{split}
\mathbf{R}\in SO(3), t\in \mathbb{R}^3 \\
C=
\begin{pmatrix}
 \mathbf{R} & t \\
 0 & 1
\end{pmatrix}
\end{split}
\end{equation}

This representation means we can compute the composition and inversion of elements in $SE(3)$ by matrix multiplication and inversion.

An element  $\delta =se(3)$ can be represented by multiples of the generators

\begin{equation}
\delta =(\mathbf{u,\omega})^T \in \mathbb{R}^6
\end{equation}

$\mathbf{u}$ is the translation, $\mathbf{u}\in \mathbb{R}^3$

$\omega$ is the rotation (exactly the axis-angle representation, its normal is the rotation angle, and its direction is the rotation axis), $\omega\in \mathbb{R}^3$

There's a 1-1 map between $SE(3)$ and $se(3)$
\begin{equation}
\begin{split}
\delta = ln(C)\\
C=exp(\delta)
\end{split}
\end{equation}

\subsection{Adjoint}
consider left-multiplication and right-multiplication in SE(3) group
\begin{equation}
C\cdot exp(\delta)=exp(Adj_C\cdot \delta) C 
\end{equation}

\begin{equation}
Adj_C=
\begin{pmatrix}
 \mathbf{R} & t_\times \mathbf{R}\\
 \bold{0} & \mathbf{R}
\end{pmatrix}
\end{equation}

\textbf{c.f. Skew-symmetric matrix of a vector}
$\alpha:=[a,b,c]^T,\beta:=[l,m,n]^T$
\begin{equation}
\begin{split}
\alpha\times \beta=
\begin{bmatrix}
 bn-cm\\
cl-an\\
am-bl
\end{bmatrix}
=
\begin{bmatrix}
 0&-c&b\\
c&0&-a\\
-b&a&0
\end{bmatrix}
\begin{bmatrix}
l\\m\\n
\end{bmatrix}
\label{skew-sym}
\end{split}
\end{equation}
So we define $\alpha_\times([\alpha]_\times)$  as the skew-symmetric matrix in $\ref{skew-sym}$

\subsection{Interpolation}

two elements $a,b\in G$, we would like to interpolate between the two elements according to a parameter $t\in [0,1]$, define an interpolation function
\begin{equation}
f:G\times G\times \mathbb{R} \rightarrow G
\end{equation}
First define a group element that tasks $a$ to $b$
\begin{equation}
d:=b\cdot a^{-1}\\
d\cdot a=b
\end{equation}
Compute the corresponding Lie algebra vector and scale it by $t$

$\mathbf{d}(t)=t\cdot ln(d)   ;d_t=exp(\mathbf{d}(t))$
\begin{equation}
f(a,b,t)=d_t\cdot a  
\end{equation}

\subsection{Gaussian Distribution}
Consider a Lie group $G$ and its Lie algebra vector space $\mathfrak{g}$, with $k$ DoF. A mean transformation $\mu\in G$ and a covariance matrix $\Sigma \in \mathbb{R}^{k\times k}$. We can sample an element from the Gaussian distribution on $G$
\begin{equation}
\begin{split}
\delta \sim \mathcal{N}(0;\Sigma)(\delta \in \mathfrak{g})\\
x=exp(\delta)\cdot \mu 
\end{split}
\end{equation}
c.f. Gaussian in $\mathbb{R}^D$
\begin{equation}
N(\mathbf{x} \mid \mu, \boldsymbol{\Sigma})=\frac{1}{(2 \pi)^{D / 2}} \frac{1}{|\boldsymbol{\Sigma}|^{1 / 2}} \exp \left\{-\frac{1}{2}(\mathbf{x}-\mu)^{T} \boldsymbol{\Sigma}^{-1}(\mathbf{x}-\mu)\right\}
\end{equation}

\section{Experiments showing $p_1$-like transition is easier to learn}
\label{appd:exp_p1}
\section{Implementation of \SE equivariant and invariant backbones}
\label{appd:backbone}

\section{Equivariant Diffusion on SE(3) manifold}
\label{appd:EquiDiff}
\subsection{Add Noise}
\label{appd:EquiDiff-adnoise}

\href{https://ieeexplore.ieee.org/abstract/document/10161569}{SE(3)-DiffusionFields: Learning smooth cost functions for joint grasp and motion optimization through diffusion} propose a diffusion process on SE(3) method

$\mathbf{H}\in SE(3)$

Add noise
\begin{equation}
\hat{\boldsymbol{H}}=\boldsymbol{H} \operatorname{exp}(\boldsymbol{\delta}), \boldsymbol{\delta} \sim \mathcal{N}\left(\mathbf{0}, \sigma_{k}^{2} \boldsymbol{I}\right)
\end{equation}

Denoise
\begin{equation}
\boldsymbol{H}_{k-1}=\operatorname{exp}\left(\frac{\alpha_{k}^{2}}{2} \boldsymbol{s}_{\boldsymbol{\theta}}\left(\boldsymbol{H}_{k}, k\right)+\alpha_{k} \boldsymbol{\epsilon}\right) \boldsymbol{H}_{k}
\end{equation}
\textbf{c.f. Sampling with Langevin Dynamics}
\begin{equation}
x_{k-1}=x_k+\frac{\alpha_k^2}2s_{\boldsymbol{\theta}}(x_k,k)+\alpha_k\epsilon , \epsilon\sim\mathcal{N}(\boldsymbol{0},\boldsymbol{I}) 
\end{equation}

\subsection{SE(3) Equivariant Diffusion for an Action Sequence}

\textbf{c.f. \href{https://diffusion-policy.cs.columbia.edu/}{Diffusion Policy}}
\begin{equation}
\mathbf{A}_{t}^{k-1}=\alpha(\mathbf{A}_{t}^{k}-\gamma \varepsilon_{\theta}\left(\mathbf{O}_{t}, \mathbf{A}_{t}^{k}, k\right)+\mathcal{N}\left(0, \sigma^{2} I\right))
\end{equation}
$\mathbf{A}$ is an action sequence.

\textbf{c.f. \href{https://kexue.fm/archives/9181}{DDIM}}
\begin{equation}
x_{t-1}=\frac{1}{\alpha_t}(x_t-(\bar{\beta}_t-\alpha_t\bar{\beta}_{t-1})\epsilon_\theta(x_t,t))
\end{equation}
A deterministic transformation from any noise vector to an image

In our setting, we define $A$ as a series of 6D pose of end effector. $A\in \mathbb{R}^{4\times4\times T_p}$, $4\times 4$ means homogeneous matrix, $T_p$ is the prediction horizon.

Namely $A=[H_0,H_1,...,H_{T_p}]$, each $H_i\in \mathbb{R}^{4\times 4}$

Denoising process
\begin{equation}
\hat{A}_t^{k-1}=s_\theta (\mathbf{O_t},A_t^k,k)*A^k_t\\
\label{denoise}
\end{equation}
$s_\theta$ is a series of noises in SE(3), $s_\theta=[\epsilon_0,\epsilon_1,...,\epsilon_{T_p}]$, each $\epsilon_i\in \mathbb{R}^{4\times 4}$

The $*$ operation in $\ref{denoise}$ means:
$$
s_\theta * A = [\epsilon_0 H_0,\epsilon_1 H_1,...,\epsilon_{T_p} H_{T_p}]
$$
i.e. For each action in the trajectory, our model predicts a SE(3) transformation to denoise it.

Let's consider Equiv property

when the object is transformed $\mathbf{O_t}\rightarrow T\mathbf{O_t}$

We suppose the noise-free action sequence should be $\mathbf{A}_t^0\rightarrow T\mathbf{A}_t^0$ (apply the transformation $T$ on all elements of $\mathbf{A}^0_t$)

Consider a 2-step process. i.e. $\mathbf{A}_t^2$ is sampled from Gaussian of Lie group, here we assume only transforming $\mathbf{O_t}$, such that $\mathbf{A}_t^2$ keeps unchanged.

\begin{equation}
\boldsymbol{A}^{0}_t =s_\theta(\mathbf{O_t,A_t^1},1)*s_\theta(\mathbf{O_t,A_t^2},2)*\boldsymbol{A}^{2}_t
\label{before_trans}
\end{equation}
by equivariance, we suppose 
\begin{equation}
T\boldsymbol{A}^{0}_t =s_\theta(\mathbf{TO_t,A_t^1},1)*s_\theta(\mathbf{TO_t,A_t^2},2)*\boldsymbol{A}^{2}_t
\label{after_trans}
\end{equation}
Compare $\ref{before_trans},\ref{after_trans}$, we have
\begin{equation}
Ts_\theta(\mathbf{O_t,A_t^1},1)*s_\theta(\mathbf{O_t,A_t^2},2)*\boldsymbol{A}^{2}_t\\
=s_\theta(\mathbf{TO_t,A_t^1},1)*s_\theta(\mathbf{TO_t,A_t^2},2)*\boldsymbol{A}^{2}_t
\label{equiv_prop}
\end{equation}
We can design 
\begin{equation}
\begin{split}
s_\theta(\mathbf{O,A},k)=
\left\{\begin{matrix}
s_{\theta,e}(\mathbf{O,A},k),k=1
 \\
s_{\theta,i}(\mathbf{O,A},k),k>1
\end{matrix}\right.
\end{split}
\end{equation}
divide the noise into an invariant branch and an equivariant branch 
\begin{equation}
\begin{split}
s_{\theta,i}(\mathbf{O,A},k)=s_{\theta,i}(T\mathbf{O,A},k)\\
Ts_{\theta,e}(\mathbf{O,A},k)=s_{\theta,e}(T\mathbf{O,A},k)\\
\end{split}
\end{equation}
such that the LHS and RHS of $\ref{equiv_prop}$ are equal.

\crtie{The input and output can be tuned according to experiment results}
In practice, for the input point cloud $\mathbf{O}\in\mathbb{R}^{N\times 6}$(xyz,rgb), we treat rgb as three type-0 features. We consider $\mathbf{A}$ as a set of type-0 features ($16\times T_p$) and $k$ is a type-0 feature. So the input of both branches is xyz and $3+16\times T_p +1$ type-0 features.

As for the output, the equivariant branch should output $3\times T_p$ type-1 vectors for rotation and $3\times T_p$ type-0 scalar for translation; the invariant branch should output $4\times 3\times T_p$ type-0 scalars. Here we get a SE(3) transformation \textbf{for each point}. 

How to aggregate? The simplest way is to compute \textbf{weighted sum} over all points. 

\subsection{Loss function design}

\href{https://openreview.net/pdf?id=BY88eBbkpe5}{DDPM on SO(3) manifold}

\href{https://proceedings.neurips.cc/paper_files/paper/2023/file/43069caa6776eac8bca4bfd74d4a476d-Paper-Conference.pdf}{SE(3) Diffusion Model for pose estimation}

\textbf{c.f. \href{https://kexue.fm/archives/9119}{DDPM}}
\begin{equation}
\left\|\varepsilon-\boldsymbol{\epsilon}_{\boldsymbol{\theta}}\left(\bar{\alpha}_{t} \boldsymbol{x}_{0}+\bar{\beta}_{t} \varepsilon, t\right)\right\|^{2}
\end{equation}

% SE(3) diffusion formula
% \begin{equation}
%     \mathbf{H}_{t}=\underbrace{\operatorname{Exp}\left(\gamma \sqrt{1-\bar{\alpha}_{t}} \varepsilon\right)}_{\text {Perturbation }} \underbrace{\mathcal{F}\left(\sqrt{\bar{\alpha}_{t}} ; \mathbf{H}_{0}, \mathbb{H}\right)}_{\text {Interpolation }}, \varepsilon \sim \mathcal{N}(\mathbf{0}, \mathbf{I})
% \end{equation}

% $\mathcal{F}$ is a interpolation function.$\mathbb{H}$ is the identity element in $SE(3)$
% \begin{equation}
% \mathcal{F}\left(\sqrt{\bar{\alpha}_{t}} ; \mathbf{H}_{0}, \mathbb{H}\right)=\operatorname{Exp}\left(\left(1-\sqrt{\bar{\alpha}_{t}}\right) \cdot \log \left(\mathbb{H} \mathbf{H}_{0}^{-1}\right)\right) \mathbf{H}_{0}
% \end{equation}

In our setting, when adding noise, we have
\begin{equation}
    A_t^k = \varepsilon^{-1} * A_t^{k-1}
    \label{addnoise}
\end{equation}
where $\varepsilon$ is a series of random noises, each noise is drawn from Gaussian distribution on SE(3) . Rewriting \ref{addnoise}
as $A_t^{k-1} = \varepsilon * A_t^k$
When denoising, we have \ref{denoise}, 
$$
\hat{A}_t^{k-1}=s_\theta (\mathbf{O_t},A_t^k,k)*A^k_t\\
$$

We aim to minimize the distance between $A_t^{k-1}$ and $\hat{A}_t^{k-1}$. Equivalently, we minimize distance between $s_\theta$ and $\varepsilon$.
We can respectively compute the rotation part and translation part, denote the rotation part of $\varepsilon$ and $s_\theta$ as $R,\hat{R} \in T_p\times SO(3)$, translation part as $t,\hat{t} \in T_p\times \mathbb{R}^3$. We supervise the geodesic distance between each SO(3) element of $R,\hat{R}$; L2 loss of $t,\hat{t}$

\textbf{c.f. Geodesic Distance between rotations.}
One can refer to \href{http://boris-belousov.net/2016/12/01/quat-dist/}{this blog} for the definition of geodesic distance on different representations of SO(3) group.

% 理论上更好
% 有的东西不能被6d pose来描述，我们的更通用
% 不需要显式pose 
% deformable 就没法pose estimation

\section{True SE(3) Invariant \& Equivariant modules}
In general, each module consists of 2 SE(3) transformer backbones, called as \textit{pos\_net} and \textit{ori\_net}, predicting translation and rotation.

\subsection{Invariant module}
We let \textit{pos\_net} predict 3 type0 feature, which is naturally invariant to any SE(3) transformation of the pointcloud.

We let \textit{ori\_net} predict 6 type0 features, and then implement Schimidt orthogonalization to get rotation matrix. As the 6 type0 features are SE(3) invariant, the rotation matrix is also invariant.

\subsection{Equivariant module}

We let \textit{ori\_net} predict 2 type1 features, and then implement Schimidt orthogonalization to get rotation matrix. As the 2 type1 features are SE(3) equivariant, the rotation matrix is also equivariant.

We let \textit{pos\_net} predict 2 type1 feature and 3 type0 feature(denoted as \textit{offset}). First we implement Schimidt orthogonalization on the 2 type1 feature, get a rotation matrix (denoted as $R$). Additionally, we denote the mass center of the input point cloud as $\mathcal{M}:=\frac{1}{N}\Sigma_{i=1}^{N}x_i$, $x_i$ is the coordinate of the $i-th$ point. Then we can write the predicted translation $t$ as 
\begin{equation}
    t(\mathcal{X})=\mathcal{M} + R\cdot \textit{offset}
\end{equation}

We can prove this translation vector is equivariant to any SE(3) transformation of the input pointcloud. When the input point cloud is transformed, $\mathcal{X}`=R_{data}\mathcal{X}+t_{data}$. 
\begin{equation}
\begin{split}
t`(\mathcal{X})=(R_{data}\mathcal{M}+t_{data})+ R_{data}R\cdot \textit{offset}\\
=R_{data}(\mathcal{M} + R\cdot \textit{offset})+t_{data} \\
=R_{data} t(\mathcal{X})+t_{data}
\end{split}
\end{equation}


\section{Simulation Tasks– Further Details}
\label{appd:SIMULATION TASKS}
\textbf{Unscrew bottle cap.}
In this task, the demonstrations show robots Unscrewing bottle cap with parallel gripper. Success in this task depends on whether the bottle cap is successfully opened.


\textbf{Open door.}
we initialize the gripper at a point p sampled on the handle of the door and set the forward orientation along the negative direction of the surface normal at p. And then we pull the door by a degree. Different from door pushing, we perform a grasping at contact point p for pulling.

\textbf{Rotate Triangle.}
In this task, a 2D anchor pushes a Triangle shaped object on a plane. The task reward is computed as the percentage of the Triangle shape that overlaps with the target Triangle pose.

\textbf{Calligraphy.}
In this task, the demonstrations involve robots executing precise and elegant strokes with a calligraphy pen. Success in this task is determined by the aesthetic quality and accuracy of the characters or patterns formed, which should closely resemble the target trajectory.

\textbf{Cloth Folding and Fling.}
Folding that folds garments. A folding succeeds when the  Intersection-over-Union (IOU) between the target and the folded garments exceeds a bar \citep{xue2023unifold,clothfunnel2022canberk}. Fling denotes garment initial states  are generated by flinging (more realistic).

==> tex/Limit.tex <==
\textcolor{red}{
\section{Limitation}
This paper proposes an efficient \SE equivariant diffusion policy to address a class of robotic manipulation tasks with specific symmetries. 
However, the proposed method has certain limitations.
% We clarify two assumptions of this paper.
1) The equivariance of \ours\ is designed for object point clouds, so, pre-processing is required to extract segmented object point clouds from the scene point clouds.
2) The action space is defined as the 6D poses of the end-effectors, and we assume the end-effectors can reach any feasible 6D pose by Inverse Kinematics solvers and controllers.
Additionally, this action space is not able to tackle dexterous manipulation tasks as they need action space with higher dimension.
}
